EqFix: Fixing LaTeX Equation Errors by Examples

LaTeX is a widely-used document preparation system. Its powerful ability in mathematical equation editing is perhaps the main reason for its popularity in academia. Sometimes, however, even an expert user may spend much time fixing an erroneous equation. In this paper, we present EqFix, a synthesis-based repairing system for LaTeX equations. It employs a set of fixing rules and can suggest possible repairs for common errors in LaTeX equations. A domain-specific language is proposed for formally expressing the fixing rules. The fixing rules can be automatically synthesized from a set of input-output examples. An extension of relaxers is also introduced to enhance the practicality of EqFix. We evaluate EqFix on real-world examples and find that it can synthesize rules with high generalization ability. Compared with a state-of-the-art string transformation synthesizer, EqFix solved 37% more cases and spent less than half of their synthesis time.

==> Makefile <==
SAMPLES = \
	paper.tex

CHAPTERS = $(filter-out paper.tex, $(wildcard *.tex))

BIB = *.bib

PDF = ${SAMPLES:%.tex=%.pdf}

all: ${PDF}

%.pdf: %.tex $(CHAPTERS) custom.sty $(BIB)
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	pdflatex -synctex=1 -interaction=nonstopmode $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF)


==> implementation.tex <==
\section{The EqFix System}\label{sec:impl}

We prototyped the proposed approach as a tool \EqFix, written in a combination of F\# and C\#, running on .NET core platform.
Rule application, synthesis algorithms and relaxer extensions were built from scratch 
following the approaches proposed in the paper.
We developed the synthesizer for the string transformation language $\mathcal{L}_\text{ST}$ under PROSE\footnote{https://github.com/Microsoft/prose} framework (proposed in \cite{flash-meta}),
in which we specified the syntax and semantic of our DSL,
a set of witness functions for guiding PROSE's synthesis engine,
and a set of scoring functions for ranking candidate programs.

\EqFix maintains all fixing rules learned so far in a \emph{rule library}.
This is indeed necessary, as we need different rules to solve a variety of different repairing tasks in practice.
\EqFix supports two running modes -- \emph{training mode} and \emph{applying mode}.
In the training mode, \EqFix learns a set of rules from user-provided examples,
and record them in the rule library.
For implementation reason, it is impractical and inefficient to store all candidate fixing rules.
Instead, we only store the top-ranked rules, using a user-specified rank $k$ (default 10), indicating the top-$k$ rules will be stored.

In the applying mode, an end user requests to repair an erroneous equation.
\EqFix searches in its rule library for all applicable rules, i.e. those whose error patterns can match against the error message, and attempts to apply them to the input equation.
If the fixing result is approved, then we are done.
Otherwise, \EqFix attempts the next applicable rule and the above interaction repeats.
It fails if (1) no applicable rules are found, or (2) all suggested results are rejected by the end user.
In either case, we expect an expert user to figure out a correction, which,
in association with the erroneous equation and the error message,
form a new example.
This new example can then be fed to \EqFix for incrementally learning a new rule to enlarge the rule library, by which several new equation repair problems (belonging to the same type) may be solved in future.

Error patterns are allowed to be incrementally inserted into the rule library, which makes it possible for users to extend their own keywords if a new error type is yet not covered by the rule library.
To achieve this, they simply prepare a set of examples, where they specify the error messages directly using the new keywords, and feed them to \EqFix for training.
The error pattern of the synthesized rules can match the new keywords.

Furthermore, we believe that \EqFix can gain benefit from \emph{source-crowded learning},
a technique that has been adopted in many synthesis applications such as \cite{error-messages,Crowd-Sourcing,Code-Feedback,NoFAQ},
where unsolved problems are published on the web and expert users are invited to post their solutions.
Combining \EqFix's incremental rule library design with source-crowded learning,
a large rule library would be established and the power of \EqFix at solving equation repair problems would be significantly augmented.

